FEASTS Combined with Interferometry (IV): Mapping HI Emission to a limit of $N_{\text{HI}}=10^{17.7} \text{cm}^{-2}$ in Seven Edge-on Galaxies

We present a statistical study of the neutral atomic hydrogen (HI) gas extending into the circumgalactic medium perpendicular to the disk for 7 edge-on galaxies with inclinations above $85^{\circ}$ from the FEASTS program with a $3\sigma$ ($20\,\text{km}\,\text{s}^{-1}$) column density ($N_{\text{HI}}$) depth of $5\times10^{17} \text{cm}^{-2}$. We develop two photometric methods to separate the extraplanar HI from the disk component, based on existing interferometric data and parametric modeling of the disk flux distribution respectively. With both methods, the FEASTS data exhibit clear extended wings beyond the disk along the minor axis. The extraplanar HI accounts for 5% to 20% of the total HI mass and extends to $20\text{-}50$ kpc at $N_{\text{HI}}=10^{18} \text{cm}^{-2}$. We find a tight positive correlation between vertical extensions of the extraplanar HI and total HI mass $M_\text{HI}$. The iso-density shape of HI at $N_{\text{HI}}=10^{18} \text{cm}^{-2}$ has an average axis ratio of $0.56\pm0.11$. The off-disk $N_{\text{HI}}$ profiles of these edge-on galaxies well represent the lower envelop of previous Lyman-$\alpha$ absorption measurements at low-redshift. Our results suggest that at $N_{\text{HI}}=5\times10^{17} \text{cm}^{-2}$, the HI extends considerably further than the known thin and thick disks in the vertical direction, but still remains much flattener than a spherical distribution, consistent with theoretical expectations that outflow, circulation, and accretion should have different impacts in these two directions. We show the tension of our results with Illustris and TNG predictions, highlighting the constraining power of our results for future simulations.

==> symb.tex <==
\makeatletter
\renewcommand\ion[2]{\texorpdfstring{\text{#1\,\textsc{\@roman{#2}}}}{#1 \@roman{#2}}}
\makeatother
\newcommand*{\HI}{\ion{H}{1}\xspace}
\newcommand*{\sbHI}[1][]{\tsb{\HI\if\relax\detokenize{#1}\relax\else,#1\fi}\xspace}
\newcommand*{\tsb}[1]{\ensuremath{_{\text{#1}}}}

\newcommand*{\RHI}[1][]{\ensuremath{R\sbHI[#1]}\xspace}
\newcommand*{\MHI}{\ensuremath{M\sbHI}\xspace}
\newcommand*{\NHI}{\ensuremath{N\sbHI}\xspace}
\newcommand*{\fHI}{\ensuremath{f\sbHI}\xspace}
\newcommand*{\MHIint}{\ensuremath{M\sbHI[int]}\xspace}
\newcommand*{\NHIlim}{\ensuremath{N\sbHI[lim]}\xspace}
\newcommand*{\sfr}{\ensuremath{\text{SFR}}\xspace}
\newcommand*{\ssfr}{\ensuremath{\text{sSFR}}\xspace}
\newcommand*{\uMsun}{\unit{\Msun}\xspace}

\newlength{\myhalfimgsize}
\setlength{\myhalfimgsize}{3.5in}
\newcommand*\myplotone[1]{%
  \centering
  \leavevmode
  \includegraphics[width={%
    \ifdim\textwidth=\linewidth%
      2\myhalfimgsize%
    \else\ifdim\linewidth>\myhalfimgsize%
      \myhalfimgsize%
    \else%
      \linewidth
    \fi\fi}]{#1}%
}%

\IfFileExists{newtx.sty}{%
    \usepackage{newtx}
  }{%
    \usepackage{newtxtext,newtxmath}
  }
  \usepackage{CJK}
  \AtBeginDocument{\DeclareSIUnit[quantity-product={}]\degree{\text{\textdegree}}}


\DeclareSIUnit\yr{yr}
\DeclareSIUnit\Gyr{\giga\yr}
\DeclareSIUnit\Myr{\mega\yr}
\DeclareSIUnit\pc{pc}
% \DeclareSIUnit\parsec{pc}
\DeclareSIUnit\Msun{M\ensuremath{_\odot}}
\DeclareSIUnit\kpc{\kilo\pc}
\DeclareSIUnit\Mpc{\mega\pc}
\DeclareSIUnit\dex{dex}
\DeclareSIUnit\deg{deg}
\DeclareSIUnit\mag{mag}
\DeclareSIUnit\jansky{Jy}
\DeclareSIUnit\beam{beam}
\DeclareSIUnit\pixel{pixel}

